CRAFT: A library for easier application-level Checkpoint/Restart and Automatic Fault Tolerance

In order to efficiently use the future generations of supercomputers, fault tolerance and power consumption are two of the prime challenges anticipated by the High Performance Computing (HPC) community. Checkpoint/Restart (CR) has been and still is the most widely used technique to deal with hard failures. Application-level CR is the most effective CR technique in terms of overhead efficiency but it takes a lot of implementation effort. This work presents the implementation of our C++ based library CRAFT (Checkpoint-Restart and Automatic Fault Tolerance), which serves two purposes. First, it provides an extendable library that significantly eases the implementation of application-level checkpointing. The most basic and frequently used checkpoint data types are already part of CRAFT and can be directly used out of the box. The library can be easily extended to add more data types. As means of overhead reduction, the library offers a build-in asynchronous checkpointing mechanism and also supports the Scalable Checkpoint/Restart (SCR) library for node level checkpointing. Second, CRAFT provides an easier interface for User-Level Failure Mitigation (ULFM) based dynamic process recovery, which significantly reduces the complexity and effort of failure detection and communication recovery mechanism. By utilizing both functionalities together, applications can write application-level checkpoints and recover dynamically from process failures with very limited programming effort. This work presents the design and use of our library in detail. The associated overheads are thoroughly analyzed using several benchmarks.

==> Makefile <==
#disable implicit rules. Necessary for correct gracebat functionality
.SUFFIXES:


L	=	pdflatex
LL =  latex
M	=	makeindex
B	=	bibtex
P	=	dvipdf
F	=	fig2dev
X	=	gracebat
D	=	dvips
DPDF	=	dvipdfm
PSPDF	=	ps2pdf
 
#.PHONY: pdf #clean distclean
.PRECIOUS: %.eps %.dvi %.ps %.png
SOURCES	= $(wildcard *.tex)   $(wildcard *.bib)

# put alls EPS and fig files in /images , e.g. some subdir
# that are generated from sources (AGR, FIG)
# by the make process

PSE_ALL=$(subst .agr,.eps,$(shell find ./images -name "*.agr"))
PSE_ALL+=$(subst .xgr,.eps,$(shell find ./images -name "*.xgr"))
PSE_ALL+=$(subst .fig,.eps, $(shell find ./images -name "*.fig"))
PSE_ALL+=$(subst .agr,.png, $(shell find ./images -name "*.agr"))
PSE_ALL+=$(subst .xgr,.png, $(shell find ./images -name "*.xgr"))

TARGET	= craft-paper

#IMAGES = ./images/Results/

pdf:	 $(TARGET).pdf
toc:
		$(LL) $(TARGET).tex
		$(LL) $(TARGET).tex


new: clean pdf


%.dvi:  $(PSE_ALL) $(TARGET).tex $(SOURCES) # $(EPSE) $(EPSR) 
	$(LL) $(TARGET).tex ; $(B) $(TARGET) ; $(LL) $(TARGET).tex ; $(LL) $(TARGET).tex

%.eps: %.fig
	$(F) -L eps $< $@

%.eps: %.agr
	$(X) -hdevice EPS -hardcopy $<  -wd $(dir $<)

%.eps: %.xgr
	$(X) -hdevice EPS -hardcopy $<  -wd $(dir $<)


%.png: %.eps
	$(X) -hdevice PNG   -hardcopy  $<  -wd $(dir $<)

	#convert $< $@
%.ps: %.agr
	$(X) -hdevice PS -hardcopy  $<

%.ps: %.dvi
	$(D) -Ppdf -o $@ $<

#%.pdf: %.dvi
#	$(DPDF) $<

%.pdf: %.ps
#	$(L) $<
	$(PSPDF) -dEmbedAllFonts=true -dSubsetFonts=true -dEPSCrop=true -dPDFSETTINGS=/prepress $<

%.latex: %.fig
	$(F)  $< $@ #-L pictex

#embedd: ijhpc08.pdf
#	gs -dBATCH -dNOPAUSE  -sOutputFile=ijhpc-embedded.pdf -dPDFSETTINGS=/prepress -dEmbedAllFonts=true -sDEVICE=pdfwrite $<

#pict: 
#	ps2pdf  images/LBM/32-192CudaLBMNonPow2Padding8800GTX.ps  images/LBM/32-192CudaLBMNonPow2Padding8800GTX.pdf
#	ps2pdf images/LBM/32-192CudaLBMNonPow2PaddingGT200.ps  images/LBM/32-192CudaLBMNonPow2PaddingGT200.pdf
#	ps2pdf  images/LowLevelBench/PCIexpress_Cuda23_GTX280.ps  images/LowLevelBench/PCIexpress_Cuda23_GTX280.pdf
##summary.pdf: summary.tex
#	$(LL) $@ && $(LL) $<
clean:
	-rm -f *.aux *.dvi *.log *.bbl $(TARGET).pdf $(TARGET).dvi $(TARGET).ps 

distclean: clean
	-rm -f *~ *.blg *.idx *.ind *.ilg *.toc #$(EPSE)

figures: figures.tex
# 	cat *.tex |grep -e "begin{figure}" -e"includegraphics" -e "end{figure}" |grep -v -e"%" |sed -e "s/...\\\columnwidth/1.0\\\textwidth/"  > figure.tex 
# 	$(LL) figures.tex
# 	$(D) -Ppdf -o  figures.ps figures.dvi
# 	$(PSPDF)  figures.ps


==> background.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

This section describes the basic building blocks of a fault tolerant program 
and defines the scope of this research contribution.

we do not rely of address sections of memory because there can be many data-types.

fault-le

CR: 
  SCR

Automatic FT:
ULFM









==> cpGhost.tex <==
\begin{lstlisting}[float,style=base,caption={The class definition for extending CRAFT support for GHOST vector data type.},label=algo:craftghostvector]
class CpGhostDenseMat: public CpBase  
{
public:
	CpGhostDenseMat(ghost_densemat *  dataPtr_, const MPI_Comm cpMpiComm_=MPI_COMM_WORLD);
	~CpGhostDenseMat(){}	
	int update();
	int write(const std::string * filename);
	int read (const std::string * filename);

private:
	ghost_densemat * dataPtr;
	ghost_densemat * asynData;
};

CpGhostDenseMat::CpGhostDenseMat(ghost_densemat *  dataPtr_, const MPI_Comm cpMpiComm_){
		asynData = new ghost_densemat[1];
		dataPtr  = new ghost_densemat[1];
	
		dataPtr   = dataPtr_;
		ghost_densemat_create(&asynData, dataPtr->context, dataPtr->traits); 
		ghost_densemat_init_densemat(asynData, dataPtr, 0, 0);
}

int CpGhostDenseMat::update(){
  ghost_densemat_init_densemat(asynData, dataPtr, 0, 0);
  return EXIT_SUCCESS;
}

int CpGhostDenseMat::write( const std::string * filename){
  asynData->toFile(asynData, (char *) (*filename).c_str(), MPI_COMM_SELF);
  return EXIT_SUCCESS;
}

int CpGhostDenseMat::read(const std::string * filename){
  asynData->fromFile(dataPtr, (char *) (*filename).c_str(), MPI_COMM_SELF);
  return EXIT_SUCCESS;
}
\end{lstlisting}

